Linking electromagnetic and gravitational radiation in coalescing binary neutron stars

We expand on our study of the gravitational and electromagnetic emissions from the late stage of an inspiraling neutron star binary as presented in Ref. \cite{Palenzuela:2013hu}. Interactions between the stellar magnetospheres, driven by the extreme dynamics of the merger, can yield considerable outflows. We study the gravitational and electromagnetic waves produced during the inspiral and merger of a binary neutron star system using a full relativistic, resistive MHD evolution code. We show that the interaction between the stellar magnetospheres extracts kinetic energy from the system and powers radiative Poynting flux and heat dissipation. These features depend strongly on the configuration of the initial stellar magnetic moments. Our results indicate that this power can strongly outshine pulsars in binaries and have a distinctive angular and time-dependent pattern. Our discussion provides more detail than Ref. \cite{Palenzuela:2013hu}, showing clear evidence of the different effects taking place during the inspiral. Our simulations include a few milliseconds after the actual merger and study the dynamics of the magnetic fields during the formation of the hypermassive neutron star. We also briefly discuss the possibility of observing such emissions.

==> myresize <==
#!/usr/bin/perl


@filelist = `find . -name "*.ps"`;

$diff = 999;

#
#
while ($entry = shift(@filelist) ) {
    chop($entry);
    #print " entry = $entry \n";
    ($base,$ext,$junk) = split(/\./,$entry);
    print " entry = $entry \n";
    #($realbase,$num,$junk) = split(/r/,$base);
    #print " realbase = $realbase \n";
    #print " num = $num \n";
    #$newnum = $num - $diff;
    #$newname = $realbase."r".$newnum."\.".$ext;
    #print " newname = $newname\n";
    #print " $entry   --->    $newname \n";
    #system('/bin/mv $entry $newname');
    system(ls -l $entry);
    $rc = `convert $entry +repage j.gif`;
    $rc = `convert j.gif +repage $entry`;
    system(ls -l $entry);
}

